Demystifying Datapath Accelerator Enhanced Off-path SmartNIC

Network speeds grow quickly in the modern cloud, so SmartNICs are introduced to offload network processing tasks, even application logic. However, typical multicore SmartNICs such as BlueFiled-2 are only capable of processing control-plane tasks with their embedded processors that have limited memory bandwidth and computing power. On the other hand, cloud applications evolve rapidly, such that a limited number of fixed hardware engines in a SmartNIC cannot satisfy the requirements of cloud applications. Therefore, SmartNIC programmers call for a programmable datapath accelerator (DPA) to process network traffic at line rate. However, no existing work has unveiled the performance characteristics of the existing DPA. To this end, we present the first architectural characterization of the latest DPA-enhanced BlueFiled-3 (BF3) SmartNIC. Our evaluation results indicate that BF3's DPA is significantly wimpier than the off-path Arm processor and the host CPU. However, we still identify that DPA has three unique architectural characteristics that unleash the performance potential of DPA. Specifically, we demonstrate how to take advantage of DPA's three architectural characteristics regarding computing, networking, and memory subsystems. Then we propose three important guidelines for programmers to fully unleash the potential of DPA. To demonstrate the effectiveness of our approach, we conduct detailed case studies regarding each guideline. Our case study on key-value aggregation achieves up to 4.3$\times$ higher throughput by using our guidelines to optimize memory combinations.

==> content/4-dsa.tex <==
\section{Benchmarking Domain-specific Engines}
\label{section_dsa}

\ming{If having to discuss the DSA, I suggest discussing how DPA and DSA interact. }

We first characterize the various domain-specific accelerators on the BF3. These engines provide a powerful computational supplement for specific applications with high processing demands. Our benchmark results indicate that these domain-specific accelerators can greatly save the required CPU core count when processing specific applications.


% Our benchmark results on these engines show that 1) hardware engines do not always provide performance gain, and 2) different engines have very different characteristics regarding throughput and latency. Rather than indiscriminately offloading workloads to engines, programmers should carefully utilize these engines according to their performance characteristics.

BF3 mainly provides the following accelerators for various applications: erasure coding, data decompression, and Regex. In the following, we compare each engine with software implementations.

\subsection{Erasure coding accelerator}
To reduce storage overhead, cloud file systems use erasure coding to replace data replication~\cite{k_earsure_coding}, at the expense of computational cost. 
Intending to become a part of cloud infrastructure, BlueField-3 provides a dedicated erasure coding accelerator.

We compare the encode and decode throughput under different data block sizes. There are three software implementations: one runs in Arm and two run in the host. One of the host implementations utilizes AVX-512~\cite{k_intel_avx} and GFNI~\cite{k_intel_gfni}. Each software implementation uses a single thread.
\ming{If comparing with an accelerator, why single-thread?}

Figure~\ref{fig_e_engine_erasure_coding} shows the encode/decode throughput. 
BF3's erasure coding engine can achieve up to 4.9$\times$/1.5$\times$ higher encode/decode throughput over the best-case software result. This indicates the huge potential of saving host cores from heavy erasure coding computation.
\ming{What testing workloads? What is the heavy erasure coding computation?}





\begin{figure}[]
    \subfloat[Encode throughput]{
        \label{fig_e_engine_ec_encode_throughput}
        \includegraphics[keepaspectratio=true, width=0.49\linewidth]{figure/e_engine_ec_encode_throughput.png}
    }
    \vspace{-1ex}
    \hspace{-2.5ex}
     \subfloat[Decode throughput]{
        \label{fig_e_engine_ec_decode_throughput}
        \includegraphics[keepaspectratio=true, width=0.49\linewidth]{figure/e_engine_ec_decode_throughput.png}
    }
    \caption{BF3 erasure coding engine vs Software implementation on Host and Arm.} 
    \label{fig_e_engine_erasure_coding}
\end{figure}

\subsection{Decompression accelerator}
To reduce storage overhead, many cloud file systems compress the data to be stored~\cite{aws_ebs,ali_oss,ali_solar,windows_azure_storage}, better decompression performance can bring better high-level application performance, especially for read-intensive workloads.

BF3 provides a powerful decompression engine. We compare it with one Arm software implementation and one host software implementation regarding throughput and latency. Both software implementation uses a single thread.

Figure~\ref{fig_e_engine_decompress} shows the decompression throughput and latency under different payload sizes. We observe that BF3 can provide up to 120$\times$ more throughput than the software implementation and reduce the latency by 14$\times$. This indicates not only the potential of saving host cores with BF3 but also the potential to reduce end-to-end file system latency.
\ming{What testing workloads? Take BF2/BF3 as an example, the decompression engine is triggered in a submission-completion style. For example, there incur BlueFlame registers ops. It would be good to go into details.}


\begin{figure}[]
    \subfloat[Decompression throughput]{
        \label{fig_e_engine_decompress_throughput}
        \includegraphics[keepaspectratio=true, width=0.49\linewidth]{figure/e_engine_decompress_throughput.png}
    }
    \vspace{-1ex}
    \hspace{-2.5ex}
    \subfloat[Decompression latency]{
        \label{fig_e_engine_decompress_latency}
        \includegraphics[keepaspectratio=true, width=0.49\linewidth]{figure/e_engine_decompress_latency.png}
    }
    \caption{BF3 decompression engine vs Software implementation on the Host and Arm.} 
    \label{fig_e_engine_decompress}
\end{figure}


\subsection{Regex accelerator}
Regular expression (Regex) matching serves as a key functionality of modern network security applications~\cite{k_regex}. It often becomes the performance bottleneck as it involves a compute-intensive scan of every received byte from the network. As such, BlueField-3 provides a powerful Regex engine to empower Regex-related applications.

We compare the Regex engine execution time with seven single-thread software implementations running in a single core of the host CPU. We use ``Learn X in Y minutes'' dataset\footnote{https://github.com/adambard/learnxinyminutes-docs} which has three traces: Email, URI, and IP.

Figure~\ref{fig_e_engine_regex} shows the BF3 Regex engine's execution time speedup over the seven software implementations. We observe that the Regex engine can provide up to 180 $\times$ speedup, indicating that the Regex engine can greatly liberate the host CPU from the intensive Regex workloads. 
\ming{How many rules you can do? What is the comparison setup?}

\begin{figure}
	\centering
	{\includegraphics[keepaspectratio=true, width=0.90\linewidth]{figure/e_engine_regex_bw_time.png}
    \vspace{-1ex}
    \caption{BF3 regex engine vs Software implementation on the host.}
    \label{fig_e_engine_regex}}
    \vspace{-1ex}
\end{figure}

\noindent{\bf Takeaways:} Utilizing the domain-specific accelerators can greatly save the host cores, programmers should consider using these accelerators as much as possible.
\ming{How should programmers use? Maybe the question is how to integrate them to the application performance path?}
